Existence results for a Cauchy-Dirichlet parabolic problem with a repulsive gradient term

We study the existence of solutions of a nonlinear parabolic problem of Cauchy-Dirichlet type having a lower order term which depends on the gradient. The model we have in mind is the following: \[ \begin{cases}\begin{split} & u_t-\text{div}(A(t,x)\nabla u|\nabla u|^{p-2})=\gamma |\nabla u|^q+f(t,x) &\qquad\text{in } Q_T,\\ & u=0 &\qquad\text{on }(0,T)\times \partial \Omega,\\ & u(0,x)=u_0(x) &\qquad\text{in } \Omega, \end{split}\end{cases} \] where $Q_T=(0,T)\times \Omega$, $\Omega$ is a bounded domain of $\mathrm{R}^N$, $N\ge 2$, $1<p<N$, the matrix $A(t,x)$ is coercive and with measurable bounded coefficients, the r.h.s. growth rate satisfies the superlinearity condition \[ \max\left\{\frac{p}{2},\frac{p(N+1)-N}{N+2}\right\}<q<p \] and the initial datum $u_0$ is an unbounded function belonging to a suitable Lebesgue space $L^\sigma(\Omega)$. We point out that, once we have fixed $q$, there exists a link between this growth rate and exponent $\sigma=\sigma(q,N,p)$ which allows one to have (or not) an existence result. Moreover, the value of $q$ deeply influences the notion of solution we can ask for. The sublinear growth case with \[ 0<q\le\frac{p}{2} \] is dealt at the end of the paper for what concerns small value of $p$, namely $1<p<2$.

==> MACRO_copia.tex <==
%--------------------------------------------------------------------
%  GREEK
%--------------------------------------------------------------------

\def\Bn{\mathcal{B}_n}
\def\B{\mathcal{B}}
\def\Vp{\Phi}
\def\b{\beta}
\def\N{\nabla}
\def\ga{\gamma}
\def\vp{\varphi}
\def\al{\alpha}
\def\om{\omega}
\def\vare{\varepsilon}
\def\eps{\varepsilon}
\def\vep{\eps}
\def\ro{\rho}
\def\te{\theta}
\def\un{u_n}
\def\hun{\hat{u}_n}
\def\unh{\hat{u}_n}
\def\vn{v_n}
\def\hvn{\hat{v}_n}
\def\vne{v_n^\eps}
\def\ve{v^\eps}
\def\hvne{\hat{v}_n^\eps}
\def\vneh{\hat{v}_n^\eps}
\def\zn{z_n}
\def\zne{z_n^\eps}
\def\zneh{\hat{z}_n^\eps}
\def\zeh{\hat{z}^\eps}
\def\tenu{\te_n(u)}
\def\up{[u]_+}
\def\vm{[v]_-}
\def\tenv{\te_n(v)}
\def\kin{\chi_{\{\un>\vn\}}}
\def\ki{\chi_{\{u>v\}}}
\newcommand{\de}{\delta}
\newcommand{\lm}{\lambda}
\newcommand{\si}{\sigma}
\newcommand{\D}{\Delta}
\newcommand{\betat}{\tilde{\beta}}
\newcommand{\sit}{\tilde{\si}}
\newcommand{\mt}{\tilde{m}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\gt}{\tilde{\ga}}
\newcommand{\car}[1]{\raise1pt\hbox{$\chi$}_{#1}}
\def\q{\quad}
\def\qq{\qquad}
\def\t{\text}

%--------------------------------------------------------------------
%  MATH
%--------------------------------------------------------------------

\newcommand{\Tnu}{T_n(u)}
\newcommand{\integrale}{\int_\Omega}
\newcommand{\meas}{\text{meas}}
\def\tS{\tilde{S}}
\newcommand{\ds}{\displaystyle}
\DeclareMathOperator{\diver}{\text{div}}
\def\dive{\text{div }}
\DeclareMathOperator{\R}{\mathbb{R}}
\DeclareMathOperator{\Na}{\mathbb{N}}
\DeclareMathOperator{\rn}{\R^N}
\def\og{\leavevmode\raise.3ex\hbox{$\scriptscriptstyle\langle\!\langle$~}}
\def\fg{\leavevmode\raise.3ex\hbox{~$\!\scriptscriptstyle\,\rangle\!\rangle$}}
\def\ra{\rangle}
\def\la{\langle}
\def\dx{d(x)}
\def\co{c_0}
\def\l{\left(}
\def\r{\right)}


%--------------------------------------------------------------------
%  COLORS
%--------------------------------------------------------------------

\definecolor{bor}{cmyk}{0.21,0.93,0.86,0.12}
\definecolor{air}{rgb}{0.178, 0.51, 0.51}
\definecolor{air2}{cmyk}{.82, 0., .67, .11}
\definecolor{range}{cmyk}{0,0.599,1,0.188}
\definecolor{range2}{rgb}{0.599,1,0.188}
\definecolor{vio}{rgb}{.4,0,.4}
\definecolor{pan}{rgb}{.17,.87,.64}
\definecolor{seagreen}{rgb}{0.18, 0.55, 0.34}

%--------------------------------------------------------------------
%  ?????
%--------------------------------------------------------------------

\def\eqref#1{(\ref{#1})}
\def\eqrefr#1{({\rm \ref{#1}})}
\def\theequation{\arabic{section}.\arabic{equation}}




